Multilingual acoustic word embeddings for zero-resource languages

This research addresses the challenge of developing speech applications for zero-resource languages that lack labelled data. It specifically uses acoustic word embedding (AWE) -- fixed-dimensional representations of variable-duration speech segments -- employing multilingual transfer, where labelled data from several well-resourced languages are used for pertaining. The study introduces a new neural network that outperforms existing AWE models on zero-resource languages. It explores the impact of the choice of well-resourced languages. AWEs are applied to a keyword-spotting system for hate speech detection in Swahili radio broadcasts, demonstrating robustness in real-world scenarios. Additionally, novel semantic AWE models improve semantic query-by-example search.

==> background/a_section.tex <==
\graphicspath{{figures/}}

\mysection{Unimodal few-shot learning}{Unimodal Few-Shot Learning}
\label{sec:unimodal_few-shot_learning}

Some text. 
\mydefinition{An apple}{is a type of fruit.} 
Some more text.
Then a figure which will be placed either at the top or bottom of a page.

\begin{figure*}[tb]
	
	\begin{minipage}[htb!]{1.0\textwidth}
		\centering
		\includegraphics[width=\textwidth]{buckeye_cropped.pdf}
		%		\vspace*{-6pt}
	\end{minipage}
	\caption{Isolating the words in the conversational spoken sequences of the Buckeye corpus.}
	\label{fig:buckeye}
	
	%	\vspace*{-5pt}
\end{figure*}

\subsection[Siamese neural networks]{Siamese Neural Networks}
\label{sec:siamese}

Check the tex file on how to define a nomenclature item like $\boldsymbol{\mathrm{z}}^{(i)}$ \nomenclature[v]{$\boldsymbol{\mathrm{z}}^{(i)}$}{A feature representation.} or $\boldsymbol{\mathrm{x}}_{\textrm{pair}}$\nomenclature[v]{$\boldsymbol{\mathrm{x}}_{\textrm{pair}}$}{A pair of $\boldsymbol{\mathrm{x}}$.}.
You can define the nomenclature variables when you first define it. Use ``v'' for variables, ``f'' for functions and ``c'' for constants.

Then you can do some math like a triplet loss: 
\begin{equation}
\begin{split}
l_{\textrm{triplet}}(\boldsymbol{\mathrm{x}}, \boldsymbol{\mathrm{x}}_{\textrm{pair}}, \boldsymbol{\mathrm{x}}_{\textrm{neg}}) & = \mathrm{max}\{0, m+d(\boldsymbol{\mathrm{x}}, \boldsymbol{\mathrm{x}}_{\textrm{pair}})-d(\boldsymbol{\mathrm{x}}, \boldsymbol{\mathrm{x}}_{\textrm{neg}})\},
\end{split}	
\end{equation} 
where 
\begin{equation}
\begin{split}
d(\boldsymbol{\mathrm{x}}_{1}, \boldsymbol{\mathrm{x}}_{2}) & = \begin{Vmatrix}\boldsymbol{\mathrm{z}}_{1} - \boldsymbol{\mathrm{z}}_{2}\end{Vmatrix}_2^2 \\
& = \begin{Vmatrix}f_{\boldsymbol{\Theta}}(\boldsymbol{\mathrm{x}}_{1}) - f_{\boldsymbol{\Theta}}(\boldsymbol{\mathrm{x}}_{2})\end{Vmatrix}_2^2
\end{split}	
\end{equation} is the squared Euclidean distance between the embeddings $\mathbf{z}_1$ and $\mathbf{z}_2$ corresponding to $\mathbf{x}_1$ and $\mathbf{x}_2$ and $m$ is some margin parameter~\cite{wang_learning_2014,hermann_multilingual_2014}.

\section{Using the acro package}
\label{sec:acro}

Define the acronyms in the \verb+fronmatter/define_acronyms.tex+ file. 

\begin{table}[!h]
	\renewcommand{\arraystretch}{1.1}
	\centering
	\caption{This table shows the different possible commands to use with acronyms.}
	\begin{tabularx}{\linewidth}{@{}llll@{}}
		\toprule
		& \multicolumn{3}{C}{Output of acro commands for acronyms when the acronyms are used for the first time. The actual acronym form is given by the ``long'' form specified in \verb+\DeclareAcronym+.} \\
		\cmidrule(lr){2-4}
		Command    & \acl{CAE} & \acl{MTriplet}\\
		\midrule 
		\acresetall
		\verb+\ac+ & \ac{CAE} & \ac{MTriplet}\\
		\acresetall
		\verb+\Ac+ & \Ac{CAE} & \Ac{MTriplet}\\
		\acresetall
		\verb+\acl+ & \acl{CAE} & \acl{MTriplet}\\
		\acresetall
		\verb+\Acl+ & \Acl{CAE} & \Acl{MTriplet}\\
		\acresetall
		\verb+\acf+ & \acf{CAE} & \acf{MTriplet}\\
		\acresetall
		\verb+\Acf+ & \Acf{CAE} & \Acf{MTriplet}\\
		\acresetall
		\verb+\acp+   & \acp{CAE} & \acp{MTriplet}\\
		\acresetall
		\verb+\Acp+ & \Acp{CAE} & \Acp{MTriplet}\\
		\acresetall
		\verb+\acfp+ & \acfp{CAE} & \acfp{MTriplet}\\
		\acresetall
		\verb+\Acfp+ & \Acfp{CAE} & \Acfp{MTriplet}\\
		\acresetall
		\verb+\aca+ & \aca{CAE} & \aca{MTriplet}\\
		\bottomrule
	\end{tabularx}
	\label{tbl:acro_first_time_examples}
\end{table}
\newpage
\begin{table}[!h]
	\renewcommand{\arraystretch}{1.1}
	\centering
	\caption{This table shows the different possible commands to use with acronyms.}
	\begin{tabularx}{\linewidth}{@{}llll@{}}
		\toprule
		& \multicolumn{3}{C}{The output of acro commands for each subsequent use (after the first use).} \\
		\cmidrule(lr){2-4}
		Commands    & \acl{AE} & \acl{MTriplet}\\
		\midrule 
		\verb+\ac+ & \ac{CAE} & \ac{MTriplet}\\
		\verb+\Ac+ & \Ac{CAE} & \Ac{MTriplet}\\
		\verb+\acf+ & \acf{CAE} & \acf{MTriplet}\\
		\verb+\Acf+ & \Acf{CAE} & \Acf{MTriplet}\\
		\verb+\acp+   & \acp{CAE} & \acp{MTriplet}\\
		\verb+\Acp+ & \Acp{CAE} & \Acp{MTriplet}\\
		\verb+\acfp+ & \acfp{CAE} & \acfp{MTriplet}\\
		\verb+\Acfp+ & \Acfp{CAE} & \Acfp{MTriplet}\\
		\bottomrule
	\end{tabularx}
	\label{tbl:acro_subsequent_time_examples}
\end{table}

==> background/awes.tex <==
\mysection{Acoustic word embeddings}{Acoustic Word Embeddings}
\label{sec:background_awe}


This section aims to familiarise the reader with acoustic word embeddings (AWEs).
Firstly, we want to make a clear distinction between textual word embeddings and AWEs.
Textual word embeddings\footnote{From now we refer to textual word embeddings simply as word embeddings.}
are fixed-dimensional vector representations of written words.
The use of word embeddings is ubiquitous in modern natural language processing applications and research, where the first use of word representations dates back to 1986~\cite{rumelhart_learning_1986}.
State-of-the-art word embedding methods~\cite{mikolov_distributed_2013, pennington_glove_2014} exploit the co-occurrence statistics of words in a text corpora to learn word representations such that words with the same meaning have similar representations.
Consequently, for word embeddings, words that appear in a similar context will appear close to each other in vector space.
Furthermore, every instance of the same word will be represented by only one embedding vector.

On the other hand, AWEs are fixed-dimensional vector representations of spoken words.
AWEs are learned speech representations that capture the acoustic properties of spoken words.
In contrast to word embeddings, since every instance of a spoken word will be different due to the continuous nature of speech, the differences in speaker, channel and context results in every instance of the same spoken word to have a unique vector representation.
Ideally, instances of the same word type should appear close to each other in vector space and further away from instances of different word types.


\begin{figure}[!t]
	\centering
	\includegraphics[width=0.95\linewidth]{background/figures/text_vs_speech.pdf}
	\caption{Illustrating the difference between word embeddings (left) and AWEs (right).}
	\label{fig:text_vs_speech}
\end{figure}


In Figure~\ref{fig:text_vs_speech} we illustrate the fundamental differences between word embeddings and AWEs.
On the left of Figure~\ref{fig:text_vs_speech}, word embeddings from three words repeated throughout a text corpus are displayed in a two-dimensional vector space. 
The embedding of ``coat" is close to ``jacket" since these two words would appear in a similar context.

On the right of Figure~\ref{fig:text_vs_speech}, AWEs extracted from an example audio segment are also displayed in two-dimensional vector space.
Isolated speech segments are embedded such that each instance has a unique embedding that appears close to embeddings from instances of the same word type. 
The embeddings of speech segments ``coat" (green) is similar and also in close proximity to embeddings from word segments of ``goat" (red) since they have a similar sound.


We again summarise the main differences as follows: Word embedding models focus on learning embeddings that reflect the semantic relationship among words where instances of the same word are represented by the same embedding vector. Conversely, AWE models focus on learning embeddings that encapsulate the acoustic properties of spoken words where instances of the same spoken word are represented by unique (but similar) embeddings. 
Throughout this thesis we only consider AWEs. However, in Chapter~\ref{chap:semantic} we again touch on the subject of word embeddings.
Until then, forget word embeddings exist.



%Now that the reader are familiar with  an acoustic word embedding is, in the following section we introduce basic neural network information that we us to implement AWEs throughout this thesis.
%Thereafter the processing of speech data is described for training AWEs, and some speech applications relevant for AWE modelling and application.

Now that the reader is familiar with AWEs, in the following section we equip the reader with information on neural networks used for AWE modelling.
Thereafter, we describe the processing of speech data and highlight important zero-resource speech tasks relevant to AWEs.









%We provide an illustration of this process to fundamental differences between word embeddings and acoustic word embeddings.

%In figure x we display an example utterance with transcriptions.
%For now we are agnostic to any embedding techniques or segmentation of speech utterance to isolated words.
%First, lets consider the word embeddings, ignoring audio.
%The process involves identify unique word in text collection called forming a vocabulary set. (out of vocabulary difficulties?)
%training embedding model to create vector representations.
%Not sure about new example, can you simply use a lookup table? or should you give it as input to the model.




%As mentioned earlier, the word embeddings are semantically organised, meaning words that appear in similar context appear close to each other in vector space.
%This is generally not the case with AWE, as modelling approach takes isolated spoken segments, treats each word on its own, individual, disjoint, learning embedding of one word is not influence by any other words. More on this in Chapter x.  

  
% Implementaions of acoustic embeddings on a higher subword modelling level
%\begin{figure}[!t]
%	\centering
%	\includegraphics[width=0.95\linewidth]{background/figures/awe_complete.pdf}
%	\caption{Acoustic word embedding process.}
%\end{figure}
%
%Here we further describe an AWE in addition to the introduction chapter.
%An acoustic word embedding model maps variable-duration speech segments to fixed dimensional vector representations.
% 
%Concretely, given a speech segment $Y$ from which a sequence of acoustic speech features $X = \mathbf{x}_1, \mathbf{x}_2, \ldots, \mathbf{x}_T$  are extracted, the model produces a fixed dimensional vector representation $\mathbf{z}$.


%\subsection{Acoustic Word Embedding Models}
%\label{ssec:awe_models}

%We now look at various model architectures previously used to produce these embeddings.





%\subsection{Downsampling}
%\label{ssec:downsampling}
%
%\subsection{ClassifierRNN}
%\label{ssec:classifier}
%
%\subsection{CAE-RNN}
%\label{ssec:cae_rnn}
%
%\subsection{SiameseRNN}
%\label{ssec:siames}





==> contrastive/old_related_work.tex <==
\mysection{Related work}{Related Work}
%\label{sec:contrastive_background}
In this section, we quickly remind the reader of the state-of-the-art AWE models discussed in Section~\ref{sec:background_models}.
Here we describe each model in terms of the network structure as implemented in this chapter.
The three existing AWE models we consider are the \system{AE-RNN}, \system{CAE-RNN} and \system{SiameseRNN}.
Each AWE model employs deep neural networks built on RNNs (Section~\ref{ssec:background_rnn}).
%Here we thoroughly describe the the state-of-the-art approaches identified in Section~\ref{sec:background_models}, all of which employs deep neural networks built on RNNs (Section~\ref{ssec:background_rnn}).
%With advancements in deep learning, AWEs emerged as an alternative for measuring speech segments of different durations instead of the alignment-based DTW methods.
%In the zero-resource setting where annotated speech is not available for training models on labelled data, unsupervised approaches were researched.
%Many unsupervised AWE modelling approaches have been proposed as an alternative to DTW for calculating the similarity between speech segments of different duration. 
%Here we thoroughly describe the the state-of-the-art approaches identified in Section~\ref{sec:background_models}, all of which employs deep neural networks built on RNNs (Section~\ref{ssec:background_rnn}).
RNN-based AWE models sequentially processes a speech segment corresponding to a word $X = (\mathbf{x}_1, \mathbf{x}_2, \mathbf{x}_3, \ldots, \mathbf{x}_T)$ where each $\mathbf{x}_t$ is a frame-level acoustic feature, to produce a fixed-dimensional vector representing segment $X$.
%The RNN structure consists of one or more stacked recurrent layers, where the output of last recurrent layer at time $t$ is a representation of the input sequence until time $t$. 
%Chung et al.~\cite{chung_unsupervised_2016} were the first to propose using a sequence-to-sequence autoencoder recurrent neural network (\system{AE-RNN}) (Section~\ref{ssec:background_ae}) for learning fixed-dimensional representations of whole word speech segments.

\citet{kamper_truly_2019} show the \system{CAE-RNN} outperform the \system{AE-RNN} following the unsupervised monolingual training strategy.
We therefore do not include AE-RNN as a baseline model but use it for pretraining the the \system{CAE-RNN}.
For each model, an encoder unit process an input segment producing a fixed-dimensional output represented by the final hidden state of the last layer in a stacked LSTM structure.
Additionally, they apply a set of fully connected layers to the output of the last recurrent layer, projecting the output to a lower-dimensional vector $\mathbf{z}$.
The output of the RNN might be larger than the desired learned representation needed to learn intermediate information while processing the sequential input sequence.
Therefore, the final layer of the encoder RNN might contain redundant information not contributing to the discriminative characteristics of the learned representation.
By adding a set of fully connected layers, the representation can be transformed to be more discriminative.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The \system{AE-RNN} model of Chung et al.~\cite{chung_unsupervised_2016} uses the autoencoder setup (Section~\ref{ssec:background_ae}).
More specifically, a single recurrent layer to processes a word segment $X$, where the output of the recurrent layer $\mathbf{v}_{T}$, after processing the final acoustic feature $\mathbf{x}_T$, is given as input to another single recurrent layer producing an output sequence $Y$. 
The \system{AE-RNN} is trained by optimising the loss in Equation~\ref{eqn:ae_general_loss}.
After training, the final output of the recurrent layer $\mathbf{v}_T$ is taken as the AWE of an input segment.
%They use this model to obtain AWEs for a language without labelled data.
They train the \system{AE-RNN} using unknown isolated speech segments from a zero-resource language.
Speech data is segmented using word boundaries obtained from forced-alignments. 
Although, the \system{AE-RNN} models itself is trained in an unsupervised fashion, using word boundaries for segmentation relies on transcriptions of the zero-resource language.

%obtaining isolated words by segmenting untranscribed speech using known word boundaries does not make the process completely unsupervised.

%The encoder uses a stacked RNN to process an input speech segment $X$, the output produced by after processing the final acoustic feature $\mathbf{x}_T$, the last recurrent layers output is the representation of the entire speech segment.
%A decoder RNN is then used to reconstruct the input by taking the final output of the encoder RNN as input to produce the first output that is then fed to the used as the next input, repeating until the same number of inputs as the target output (the input) sequence length.   
%After training, for a input speech segment, the final layer of the encoder RNN is taken as the learned representation.

%Given a variable-length word segment as input, the encoder RNN produces a fixed-dimensional vector representation. 
%The decoder RNN then tries to reconstruct the input only taking the learned representation as input.


Inspired by the RNN-based \system{AE-RNN} of Chung et al.~\cite{chung_unsupervised_2016}, Settle and Livescu~\cite{settle_discriminative_2016} reproduced CNN-based models of Kamper et al.~\cite{kamper_truly_2019} using RNNs. 
%The two models called the \system{SiameseRNN} and \system{ClassifierRNN}.
%Although this triplet loss has been implemented in various work, Kamper et al.~\cite{kamper_deep_2016} were the first to use siamese networks to obtain acoustic word embeddings from whole word speech segments.
%Here they used CNNs as their base models.
%Settle and Livescu~\cite{settle_discriminative_2016} extended this work by replacing the CNN structure of Kamper with RNN uints.
%The \system{SiameseRNN} and \system{ClassifierRNN} of Settle and Livescu~\cite{settle_discriminative_2016}  
They reproduced the experimental setup of Kamper and shows an AWE model using the Siamese setup (\ref{ssec:background_siamese}) built on RNNs, outperforms the other models.
This model, the \system{SiameseRNN}, is especially better at organising embeddings of words that were not seen during training.
%the \system{SiameseRNN} outperforms its CNN-based counterpart and another classification  \system{ClassifierRNN} in a word discrimination task (Section~\ref{sec:background_evaluation}) and that the \system{SiameseRNN} is better at organising embeddings of words that were not seen during training.
%The \system{SiameseRNN} model is implemented using the Siamese network configuration (\ref{ssec:background_siamese}) with a similar embedding function as the \system{AE-RNN}.
Here they implement the embedding function using multiple recurrent layers, instead of a single recurrent layer.
Additionally, they apply a set of fully connected layers to the output of the last recurrent layer, projecting the output to a lower-dimensional vector $\mathbf{z}$.
The output of the RNN might be larger than the desired learned representation needed to learn intermediate information while processing the sequential input sequence.
Therefore, the final layer of the encoder RNN might contain redundant information not contributing to the discriminative characteristics of the learned representation.
By adding a set of fully connected layers, the representation can be transformed to be more discriminative.

They train the \system{SiameseRNN} using a weak form of supervision where word segments are grouped into unknown word types. 
This allows for triplet construction needed to optimise the loss in Equation~\ref{eqn:background_triplet}.
Again, this approach is not completely unsupervised since word boundaries are used for segmentation and words are grouped using class labels.
%Although they did not reimplement the \system{AE-RNN} with fully connected layers, they did this with the other two models to get final representations.

%The \system{SiameseRNN} are better at organising embeddings of words that were not seen during training than the \system{ClassifierRNN}.
%Probably due to the \system{SiameseRNN} that is trained to optimise the relative distances between words than the \system{ClassifierRNN} that learns softmax. (huh?)
%They specifically re-implemented the CNN-based models of Kamper et al.~\cite{kamper_deep_2016} that outperformed several other deep neural network models. One of the models is a classification network (\system{ClassifierRNN}) and the other a \system{SiameseRNN} (Section~\ref{ssec:background_siamese}). 
%They showed that the RNN-based models outperforms the CNN-based models of Kamper et al.~\cite{kamper_deep_2016}. 
%Settle and Livescu use a similar encoder RNN unit as Chung et al.~\cite{chung_unsupervised_2016}, to create vector representations but do not use the final hidden layer of the encoder RNN as the representation vector.
%Instead, the add a feed forward neural network to the final hidden layer of the encoder RNN. The final hidden layer of the encoder RNN gives input to the FFNN to produce a new latent embedding that is then fed to the decoder RNN. The output of the FFNN is taken as the new representation.  
%The final hidden layer of the encoder RNN might be larger than the desired learned representation, needed to learn intermediate "information" while processing the sequential input sequence.
%Therefore, the final layer of the encoder RNN might contain redundant information not contributing to the discriminative characteristics of the learned representation.
%By adding a set of fully connected layers we can further transform the representation to more discriminative representations.
%They trained the classifierRNN to using word labels and the Siamese use same weak form of supervision where segments are grouped into unknown word types using available word boundaries.
%Although they did not reimplement the \system{AE-RNN} with fully connected layers, they did this with the other two models to get final representations.


The \system{CAE-RNN} model presented by Kamper~\cite{kamper_truly_2019} is an extension of the \system{AE-RNN}.
%Kamper~\cite{kamper_truly_2019} presented a new AWE model, the correspondence autoencoder \system{CAE-RNN} (Section~\ref{ssec:background_cae}) that extends the \system{AE-RNN} of Chung et al.~\cite{chung_unsupervised_2016}. 
%The \system{CAE-RNN} network architecture is identical to the \system{AE-RNN} implementation in \cite{kamper_truly_2019}.
In the \system{CAE-RNN}, unlike the \system{AE-RNN}, the target output is not identical to the input, but rather an instance of the same word type (Section~\ref{ssec:background_cae}).
They were the first to use this correspondence learning technique in an encoder-decoder structure operating on whole word speech segments.
%The idea of using correspondent items on speech representation learning was first introduced by [], which operates on frame-level features.
%Kamper were the first to use this technique in an encoder-decoder architecture.
Similar to Settle and Livescu~\cite{settle_discriminative_2016}, they extended the encoder RNN structure by adding a single fully connected feed-forward layer to the output of the final output of the last recurrent layer.
Most importantly, the \system{CAE-RNN} is trained in a complete zero-resource setting.
In this setting, no word boundaries or class labels are assumed to be available.
Isolated word-like pairs are obtained by applying a UTD system (Section~\ref{sec:background_utd}) to the unlabelled speech data.
The UTD system is in itself unsupervised making the whole process unsupervised.
They showed the \system{CAE-RNN} outperforms the \system{AE-RNN} trained in the fully zero-resource setting.

Recently, Kamper et al.~\cite{kamper_improved_2021} presented a multilingual transfer (Section~\ref{ssec:multilingual}) approach for obtaining AWE for zero-resource languages.
Instead of using discovered word-like segments from the zero-resource language, they exploit labelled data from multiple well-resourced languages to train supervised multilingual models and then apply it to an unseen zero-resource language. 
%By pooling data from multiple well-resourced languages, true word pairs are used. 
The idea is that a model trained on multiple languages should learn a representation that would capture discriminative acoustic properties that generalise to any language. 
%Kamper et al.~\cite{kamper_improved_2021} use the \system{SiameseRNN} of Settle and Livescu~\cite{settle_discriminative_2016} and the \system{CAE-RNN} of Kamper~\cite{kamper_truly_2019} to 
Here they train a single multilingual \system{CAE-RNN} on true word pairs from multiple languages using the loss in Equation~\ref{eqn:cae_loss}.
The multilingual \system{SiameseRNN} optimises the loss in Equation~\ref{eqn:background_triplet} where, for an input example, a positive example is a word from the same word type in the same language and a negative an instance from a different word type from any language. 
They show, applying a multilingual model to an unseen target language, outperforms an unsupervised monolingual model trained on unlabelled data from the target language. 




%%%%%%%%%%
%Imagine a farmer wanting to get information on crop prices over her mobile phone, but only speaking a minority African language for which no labelled speech corpus exists. This could be solved using an unsupervised system that takes a spoken query, searches through a collection of recent radio broadcasts, and plays back those reports containing the query.
%
%For speech processing applications of this type, speech segments of different duration need to be compared. To do this without aligning segments (which is computationally expensive), acoustic word embedding models map variable-duration segments to vectors in a fixed-dimensional space, allowing for easy comparison. In recent work, an embedding model was developed which is trained on multiple well-resourced languages and then applied to a so-called zero-resource language -- a language for which no labelled data is available. A
%universal language embedding model of this type could be very useful since it would allow speech processing systems to be rapidly developed in a new language, enabling the type of technology as in the above example.
%
%In previous research, we focussed on improving multilingual embedding models to produce higher quality word embeddings to accomplish the task described in the intro paragraph. 
%We would like to extend this research by developing a system that plays back reports from a speech collection which are related in meaning to a spoken query and not necessarily containing the query.
%Such a system would be useful for gathering information related to a specific keyword from an untranscribed speech collection. 
%For example, given a search query "crops" the system should play back reports not only containing the word "crops" but also reports relevant to the word "crops". This is a very difficult problem which have not received much attention. 


==> frontmatter/acknowledgements.tex <==
\chapter*{Acknowledgements}
\addcontentsline{toc}{chapter}{Acknowledgements}
\makeatletter\@mkboth{}{Acknowledgements}\makeatother



%\begin{centering}
%{\LARGE``} \textit{A very long quote}\\
%\textit{from someone very important.} {\LARGE''}\\
%-- Mr M\\
%\end{centering}

==> frontmatter/declaration.tex <==
%\chapter*{Declaration}
\newpage
\thispagestyle{plain}
\addcontentsline{toc}{chapter}{Declaration}
\makeatletter\@mkboth{}{Declaration}\makeatother

\centerline{\includegraphics[width=8cm]{frontmatter/fig/SU_corporate_horizontal_with_slogan_RGB.pdf}}
%\vspace*{-25pt}

\section*{\centering Plagiaatverklaring / \textit{Plagiarism Declaration}}

\vspace*{5pt}

\begin{enumerate}
	\item Plagiaat is die oorneem en gebruik van die idees, materiaal en ander intellektuele eiendom van ander persone asof dit jou eie werk is.\\
	\textit{Plagiarism is the use of ideas, material and other intellectual property of another's work
		and to present is as my own.}
	
	\item Ek erken dat die pleeg van plagiaat 'n strafbare oortreding is aangesien dit 'n vorm van diefstal is.\\
	\textit{I agree that plagiarism is a punishable offence because it constitutes theft.}
	
	\item Ek verstaan ook dat direkte vertalings plagiaat is. \\
	\textit{I also understand that direct translations are plagiarism.}
	
	\item Dienooreenkomstig is alle aanhalings en bydraes vanuit enige bron (ingesluit die internet) volledig verwys (erken). Ek erken dat die woordelikse aanhaal van teks sonder aanhalingstekens (selfs al word die bron volledig erken) plagiaat is. \\
	\textit{Accordingly all quotations and contributions from any source whatsoever (including the internet) have been cited fully. I understand that the reproduction of text without quotation marks (even when the source is cited) is plagiarism}
	
	\item Ek verklaar dat die werk in hierdie skryfstuk vervat, behalwe waar anders aangedui, my eie oorspronklike werk is en dat ek dit nie vantevore in die geheel of gedeeltelik ingehandig het vir bepunting in hierdie module/werkstuk of 'n ander module/werkstuk~nie. \\
	\textit{I declare that the work contained in this assignment, except where otherwise stated, is my original work and that I have not previously (in its entirety or in part) submitted it for grading in this module/assignment or another module/assignment.}
\end{enumerate}

\vfill

\noindent \begin{tabularx}{1.0\linewidth}{|L|L|}
	\hline
	& \\[-10pt]
	\textbf{20111703} & \includegraphics[height=1.5cm]{frontmatter/fig/signature.png} \\
	%    \vspace{1cm}
	{Studentenommer / \textit{Student number}} & {Handtekening / \textit{Signature}} \\
	\hline
	& \\[-10pt]
	\textbf{C.\ Jacobs} & \textbf{11 August 2023} \\
	{Voorletters en van / \textit{Initials and surname}} & {Datum / \textit{Date}} \\
	\hline
\end{tabularx}

\vspace{15pt}



%%\chapter*{Declaration}
%%\addcontentsline{toc}{chapter}{Declaration}
%%\makeatletter\@mkboth{}{Declaration}\makeatother
%\newpage
%
%\begin{center}
%%	\vspace*{-40pt}
%
%    \includegraphics[width=7cm]{USlogo-top}
%    
%    {\rmfamily \bfseries \large Plagiaatverklaring / \textit{Plagiarism Declaration} \par}
%\end{center}
%{\small
%\begin{enumerate}[nolistsep]
%	\item Plagiaat is die oorneem en gebruik van die idees, materiaal en ander intellektuele eiendom van ander persone asof dit jou eie werk is.\\
%	\textit{Plagiarism is the use of ideas, material and other intellectual property of another’s work and to present is as my own.}
%	\item Ek erken dat die pleeg van plagiaat `n strafbare oortreding is aangesien dit ‘n vorm van diefstal is.\\
%	\textit{I agree that plagiarism is a punishable offence because it constitutes theft.}
%	\item Ek verstaan ook dat direkte vertalings plagiaat is. \\
%	\textit{I also understand that direct translations are plagiarism.}
%	\item Dienooreenkomstig is alle aanhalings en bydraes vanuit enige bron (ingesluit die internet) volledig verwys (erken). Ek erken dat die woordelikse aanhaal van teks sonder aanhalingstekens (selfs al word die bron volledig erken) plagiaat is. \\
%	\textit{Accordingly all quotations and contributions from any source whatsoever (including the internet) have been cited fully. I understand that the reproduction of text without quotation marks (even when the source is cited) is plagiarism}
%	\item Ek verklaar dat die werk in hierdie skryfstuk vervat, behalwe waar anders aangedui, my eie oorspronklike werk is en dat ek dit nie vantevore in die geheel of gedeeltelik ingehandig het vir bepunting in hierdie module/werkstuk of ‘n ander module/werkstuk nie. \\
%	\textit{I declare that the work contained in this assignment, except where otherwise stated, is my original work and that I have not previously (in its entirety or in part) submitted it for grading in this module/assignment or another module/assignment.}
%\end{enumerate}
%}
%\vspace{2ex}
%\begin{tabularx}{1.0\linewidth}{|C|C|}
%		\hline 
%		\Studentnumber & \vspace{0.5pt} \includegraphics[width=3.5cm]{signature.png} \\ %\includegraphics[width=1.5cm]{} with signature being an image \\
%		{\footnotesize \textbf{Studentenommer / \textit{Student number}}} & {\footnotesize \textbf{Handtekening / \textit{Signature}}} \\
%		\hline\medskip
%		\medspace\textsc{\Author} & \medspace{\selectlanguage{english} \SignedDate}  \\
%		\raggedright \vspace{0.1cm} {\footnotesize \textbf{Voorletters en van / \textit{Initials and surname}}} & \vspace{0.1 cm} {\footnotesize \textbf{Datum / \textit{Date}}} \\
%		\hline
%\end{tabularx}

==> hatespeech/asr.tex <==
\mysection{Keyword spotting with ASR}{Keyword Spotting With ASR}
\label{sec:hatespeech_asr}


As previously mentioned (Section~\ref{sec:hatespeech_related}) ASR is one of the most straightforward approaches to hate speech detection via KWS. 
Given a set of keywords, the ASR model first transcribes the audio into text, then the keywords are searched for in the resulting text~\cite{saeb+etal_interspeech2017}.
One property of this approach is that the downstream KWS performance depends on the ASR model's performance.

Typically, to train an ASR model we need audio with transcriptions from the target language.
In a low-resource setting, a lack of transcribed speech data from the target languages prohibits the fast development and deploying of ASR-based KWS systems.
Recently advancements in self-supervised representation learning allows for development of ASR systems with much less transcribed data usually required to get equal good performance.
%Self-supervised representation learning in speech refers to a technique where an model learns to extract meaningful representations or features from raw audio data without relying on explicitly labelled or annotated speech data. 
%Instead, it leverages the inherent structure and properties of the audio itself to create useful representations.



We use an ASR model from the Wav2vec 2.0 XLS-R family~\cite{baevski_wav2vec_2020, babu_xls-r_2022}.
XLS-R
% It
is a large-scale cross-lingual speech model pre-trained on half a million hours of unlabelled speech data in 128 languages (including Swahili but not Wolof).
The speech representation learned during cross-lingual pre-training improves performance for low-resource languages by leveraging data from the high-resource languages on which it is pre-trained.
Using the pre-trained model as a starting point, the model
is fine-tuned on labelled data from the language of interest.
% After an initial pre-training phase, the model is fine-tuned on labelled data from the language of interest. The speech representation learned during cross-lingual pre-training improves performance for low-resource languages by leveraging data from the high-resource languages. The model performs well even with limited amounts of labelled data.

Previous work has shown that this fine-tuning approach leads to competitive ASR performance even with limited amounts of labelled data~\cite{babu_xls-r_2022}.
In our experiments (Table \ref{tbl:awe} specifically) we show that the
sample efficiency of the XLS-R model also extends to KWS when training on just five minutes of labelled data.

% keyword spotting. The model performs competitively when fine-tuned on as little as one hour or even 5 minutes of labelled data (see Table \ref{tbl:awe}).



==> hatespeech/awe.tex <==
\mysection{Keyword spotting with multilingual acoustic word embeddings}{Keyword Spotting With Multilingual Acoustic Word Embeddings}
\label{sec:hatespeech_awe}


For a severely under-resourced language, there might not even be limited amounts of labelled data available to fine-tune a pre-trained ASR model.
In this scenario, collecting only a few spoken instances of a keyword of interest would allow for KWS through query-by-example (QbE) search~\cite{menon_fast_2018, van_der_westhuizen_feature_2022}.
% The advantage of this AWE KWS approach is that it can be applied to any unseen language and only requires a small number of spoken instances per keyword. 
% In a truly zero-resource setting, where no transcriptions are available to train/fine-tune an ASR model, query-by-example (QbE) speech search can be extended for KWS.
QbE is the task of retrieving utterances from a search corpus using a spoken instance of a keyword, instead of a written keyword.
% Utterances are retrieved based on the similarity between the acoustic representation of the query segment and
% When using multilingual AWEs as acoustic representations, the QbE system becomes completely language-independent.
% When using multilingual AWEs as an acoustic feature for matching the  

%\begin{figure}[!t]
%	% \vspace{-3mm}
%	\centering
%	\includegraphics[width=0.95\linewidth]{figures/qbe_grey.pdf}
%	\vspace{-2mm}
%	\caption{{Search utterances} ($u_1, u_2, \ldots, u_N$) are segmented and mapped to a fixed-dimensional space, along with a query segment $q$, to produce embeddings $\mathbf{z}_n^i$ and $\mathbf{z}_q$, respectively.
%		% The subscript $n$ represents a unique utterance within the search collection, and superscript $i$ represents a segment extracted from utterance $\mathbf{z}_n$.    
%		{Subsequently,} search utterances are ranked based on the shortest distance between a search segment $\mathbf{z}_n^i $ and the query vector $\mathbf{z}_q$.}
%	% \christiaan{In this example space, $d()$}
%	\label{fig:qbe_awe}
%	\vspace{-3mm}
%\end{figure}

The workings of an AWE-based QbE system are displayed in Figure~\ref{fig:qbe_awe}.
First, the search corpus is segmented into word-like segments.
% that can be compared to the query segment.
Ideally, we would like to use true word boundaries to segment each utterance in the search collection.
However, in
an under-resourced
% the zero-resource
setting, word boundaries are not available.
Therefore, we follow an exhaustive segmentation technique where utterances are split into overlapping segments of some minimum to some maximum duration~\cite{kamper_semantic_2019}.
Concretely, utterances from the search corpus ($u_1, u_2, \ldots, u_N$) are segmented to produce a set of variable-length speech segments $S = \{s_n^i\}$, where $i$ is the $i^\text{th}$ search segment extracted from utterance $n$.

A multilingual AWE model is then applied to the segmented search corpus and query segment,
mapping them to the same fixed-dimensional vector space.
% producing search embeddings $\mathbf{z}_n^i$ and query embedding $\mathbf{z}_q$.
We specifically use the CAE-RNN architecture~\cite{kamper_improved_2021, jacobs_acoustic_2021} to train a multilingual AWE model.
This model is trained using an encoder-decoder {recurrent neural network (RNN)} %RNN
structure, where the encoder takes a variable-length word segment as input to produce a fixed-dimensional output. 
The output vector of the encoder is then fed as input to a decoder RNN, which reconstructs a target that is not identical to the input but rather an instance of the same word type.
This model is trained on word pairs using labelled data from multiple languages
(but not
% and does not include
the target language).
At inference time, we take the projection of the final encoder RNN hidden state as the AWE of an input segment.
% This multilingual AWE model can be transferred and applied to any unseen language to embed word segments of arbitrary length.

Applying the AWE model to search segments $S$ and query segment $q$ produces search embeddings $\mathbf{z}_n^i$ and query embedding $\mathbf{z}_q$, respectively.
Utterances in the search corpus can then be ranked based on the segment-query distances $d(\mathbf{z}_n^i, \mathbf{z}_q)$.
We can then predict that all query-search pairs with a distance below some threshold are positive matches (this requires a threshold to be tuned on development data).
% \herman{Instead of ranking, the alternative is to make a binary decision for whether a segment contains a query by predicting that query-search pairs with a distance below some threshold are positive matches (this requires a threshold to be tuned on development data).}
% Furthermore, utterances can be labelled as containing a query segment by deciding on a threshold distance to label each query-search segment $(q, s_n^i)$, which requires tuning on development data.
With these
predictions
% labelled utterances
we can calculate common KWS metrics and compare them to those achieved by the ASR KWS systems.


\begin{figure}[!t]
	\centering
	\includegraphics[width=0.99\linewidth]{hatespeech/figures/kws_awe.pdf}
	\caption{Search utterances ($u_1, u_2, \ldots, u_N$) are segmented and mapped to a fixed-dimensional space, along with a query segment $q$, to produce embeddings $\mathbf{z}_n^i$ and $\mathbf{z}_q$, respectively.
	The subscript $n$ represents a unique utterance within the search collection, and superscript $i$ represents a segment extracted from utterance $\mathbf{z}_n$.    
	Subsequently, search utterances are ranked based on the shortest distance between a search segment $\mathbf{z}_n^i $ and the query vector $\mathbf{z}_q$.
	}
	\label{fig:kws_awe}
\end{figure}






==> hatespeech/definition.tex <==
\mysection{What is hate speech?}{What is Hate Speech?}
\label{sec:hatespeech_definition}



%% Meaning of hate speech
The definition of "hate speech" is multifaceted and subjective, leading to differing perspectives on its boundaries.
While some forms of hate speech involve direct attacks on individuals based on race, ethnicity, sexual orientation, gender, or religious affiliation, there are other underlying manifestations that can also be considered hate speech.
These include, "... attacks as violent or dehumanising speech, harmful stereotypes, statements of inferiority, expressions of contempt, disgust or dismissal, cursing and 
calls for exclusion or segregation...", outlined in Facebook's hate speech policy.
The latter can be potentially link to radicalisation towards violent extremism (more in Section~\ref{}). 
Nevertheless, regardless of how the term is defined or the issue it represents, there is a clear need for automated hate speech detection methods in certain situations. 




==> hatespeech/viakws.tex <==
\mysection{Hate speech detection via keyword spotting}{Hate Speech Detection via Keyword Spotting}
\label{sec:hatespeech_kws}
\vspace{-25pt}
Hate speech detection can be supported by using a \textit{keyword spotting} (KWS) system which can effectively search an audio corpus for a predetermined set of keywords or phrases that are indicative of hate speech.
%Such a KWS system have the potential ability to quickly scan through large amounts of audio content and flag parts of the audio that have been identified as potential markers of hate speech. 
It is important to note that a KWS system solely relying on keyword or phrase identification  may not be sufficient for comprehensive hate speech detection. 
For instance, given a keyword ``blood", a KWS system may retrieve utterances ``We must spill their blood and eradicate them from our society." and ``She donated blood to help save lives during the blood drive."
The former contains hate speech as it promotes violence and harm towards a specific group of people where the latter highlights a positive action.
Therefore, the context in which these potential hate speech markers occur should be carefully considered and analysed by domain experts.

%In the following section, we look at KWS approaches for low-resource languages where there are a lack of 
%However, monitoring hate speech on these radio broadcasts in low-resource languages is extremely challenging due to factors such as background noise, speaker variability, and the presence of accents or dialects in the audio.
%Furthermore, there is a severe lack of resources to develop hate speech detection tools specifically for radio audio in low-resource languages.



%We use the term \textit{keyword spotting} to refer to the process of searching an audio corpus using a written or spoken keyword/query. 
%Using a spoken keyword to search is also referred to in the literature as \textit{spoken term detection} or \textit{spoken term discovery}.

==> semantic/clustering.tex <==
\mysection{Clustering}{Clustering}
\label{sec:semantic_cluster}



==> semantic/implementation.tex <==
\mysection{Developmental experiments}{Developmental Experiments}
\label{sec:semantic_experiments}
In this section, we provide intermediary results for the three-step framework proposed in Section~\ref{sec:semantic_methodology}.
We first look at the acoustic embedding space (produced by the multilingual AWE model) and the clustering thereof.
We  visualise the textual word embeddings after training the Skip-gram model using unknown word labels (cluster IDs) as the text corpus. 


%\subsection[Purely acoustic embedding of speech segments]{Purely Acoustic Embedding of Speech Segments}

%Firstly, we produce AWEs for each spoken word segment in a speech collection using a pretrained multilingual model.
%Given that our dataset for this experiment is in English (see Section~\ref{sec:setup}) we use a \system{ContrastiveRNN} multilingual model trained on Xho+Ssw+Nbl+Nso+Tsn+Afr in the exact same setup as the multilingual models trained in Chapter~\ref{chap:related}.
%Note that the training languages do not include English, therefore producing the embeddings for all the speech segments can be seen as an unsupervised process.


%\begin{figure}[!t]	
%	\begin{minipage}[a]{.49\linewidth}
%		\centering
%		\centerline{\includegraphics[width=\linewidth]{semantic/figures/tsne_black.pdf}}
%		\centerline{(a) Unsupervised setting.}\medskip
%	\end{minipage}
%	\hfill
%	\begin{minipage}[a]{0.49\linewidth}
%		\centering
%		\centerline{\includegraphics[width=\linewidth]{semantic/figures/tsne_marked.pdf}}
%		\centerline{(b) Supervised setting.}\medskip
%	\end{minipage}
%	
%	\caption{t-SNE visualisation of AWEs from 35 hand-picked evaluation words with (a) no word class information compared to (b) embeddings labelled according to word type (i.e. what an ideal clustering would look like).} 
%	\label{fig:semantic_tsne}
%\end{figure}

%Applying the multilingual AWE to the segmented training set produces an acoustic space containing the embedding of each spoken word segment.
Applying the multilingual AWE model to the segmented training set produces acoustic embeddings in a fixed-dimensional space, each representing a spoken word segment.
Figure~\ref{fig:semantic_tsne} shows the t-SNE visualisation  of AWEs that belong to the 35 (out of 683) hand-picked evaluation words.
Figure~\ref{fig:semantic_tsne}~(a) reflects the unsupervised setting where we have no knowledge regarding the word type that an embedding belong to.
Figure~\ref{fig:semantic_tsne}~(b) shows the same embedding space, indicating the word type to which each embedding belong using true word labels.
Figure~\ref{fig:semantic_tsne}~(b) shows an ideal clustering scenario, where each embedding is assigned to its corresponding word type.
Note how these embeddings are grouped only based on acoustic similarity, without capturing any semantic information.

Figure~\ref{fig:semantic_tsne} clearly shows the AWE model's ability to produce AWEs discriminating between different word types.
However, the more acoustically similar word segments (from different types) are, the more difficult it is for the AWE model to distinguish between them.
For example, the embeddings produced by word segments ``running" and ``riding" (marked inside the red circle) are similar in sound and therefore somewhat indistinguishable.
This is illustrated by their embeddings appearing close to each other in vector space.
Evidently, any clustering method would struggle to distinguish these embeddings from each other.
%A more sophisticated AWE model might deliver higher quality AWE being able to distinguish more between word types.




%In the zero-resource setting, we don't have access to class labels, however, we exploit the 
%topology of the acoustic embedding space to infer unknown labels to embeddings.
%Since embeddings from the same word type should have similar embeddings, and be less similar than embeddings from different word types, we apply an unsupervised clustering technique to group the embeddings into different unknown classes.



%If class labels were available, each embedding could be assigned to its respective class and you would have the same setup for training word embeddings, knowing which AWE belongs to which word type.
%Because these labels are not available, we can infer them by exploiting the similarity between AWE from the same word type.

%We use the multilingual model described in Section x to produce AWE for all word segment from utterances in the training set.
%For each of the hand-picked evaluation words, we display the roduced by the AWE.
%The t-SNE visualisation the hand-picked evaluation words are displayed in Figure~\ref{fig:semantic_tsne}.
%The right side of Figure~\ref{fig:semantic_tsne} shows to which class each embedding belong (indicated by colour) using word labels. 

%On the left of Figure~\ref{fig:semantic_tsne}, illustrates the unsupervised setting where word labels are not available.

%We again use t-SNE to map the high dimensional embeddings to a lower dimensional space, illustrated in Figure~\ref{fig:semantic_tsne}.
%We select a few word examples that would illustrate the semantic relationship between words that we observe later on. 
%Important, the embeddings are colour coded for display purposes only, the class labels have is not available for clustering.
%From Figure~\ref{fig:semantic_tsne} we see that 
%Note how these embeddings are grouped together based on acoustic similarity.
%Embeddings from the same word type are grouped together.
%Because the pronunciation of some words for example ``running" and ``riding" are very similar, their AWE appear to more similar than words with more distinctive sounds (dependent on the articulation of speakers).
%However, ideally, this words should be more separated in embedding space.

%\subsection[K-Means clustering]{K-Means Clustering}
%%\label{ssec:}
%
%
%
%Applying $K$-means clustering to the acoustic embedding space assigns each embedding to one of $K$ clusters as illustrated in Figure~\ref{fig:semantic_clustered}~(b), where clusters are indicated by colour.
%Ideally, we would like all embeddings from the same word type to be assigned to a single cluster. 
%However, most embeddings from the same word type are assigned to multiple clusters (compare Figure~\ref{fig:semantic_tsne}~(b) with Figure~\ref{fig:semantic_clustered}~(b)).
%To give some perspective, the 35 hand-picked evaluation word-types are assigned to $444$ different clusters (out of 700).
%Moreover, embeddings from different word types could also be assigned to the same cluster.
%Instead of only visualising the partitioned embedding space, we evaluate the cluster quality in a more sophisticated way by calculating the cluster purity.
%Cluster purity is calculated as follows~\cite{manning_introduction_2008}: Each cluster is assigned to the class which is most frequent in the cluster, and then the accuracy of this assignment is measured by counting the number of correctly assigned items and dividing by the total number of items.
%Formally, with $K$ clusters and $M$ different classes we calculate the purity as follows:



%\begin{figure}[!t]	
%	\begin{minipage}[a]{.49\linewidth}
%		\centering
%		\centerline{\includegraphics[width=\linewidth]{semantic/figures/tsne_black.pdf}}
%		\centerline{(a) Before clustering.}\medskip
%	\end{minipage}
%	\hfill
%	\begin{minipage}[a]{0.49\linewidth}
%		\centering
%		\centerline{\includegraphics[width=\linewidth]{semantic/figures/kmeans_clustered.pdf}}
%		\centerline{(b) After clustering.}\medskip
%	\end{minipage}
%	
%	\caption{t-SNE visualisation of AWEs from 35 hand-picked evaluation words (a) before clustering and (b) after applying $K$-means clustering.} 
%	\label{fig:semantic_clustered}
%\end{figure}


%\begin{equation}
%	\begin{aligned}
%		\text{Purity} &= \frac{1}{N} \sum_{k = 1}^K \left[ \max_{m = 1}^M \left(\text{\# items in cluster $k$ from class $m$} \right)\right]	\\
%		&= \frac{1}{N} \sum_{k = 1}^K \left[ \max_{m = 1}^M \left(\sum_{i \in C_k} 1\left\{ y^{(i)} = m \right\} \right) \right]
%	\end{aligned}
%	\label{eqn:purity}
%	%	\textrm{Purity} = \frac{1}{N} \sum_{K}^{k=1 }  \text{max}_{m=1} 
%\end{equation}
where $1 \{\cdot\}$ is a indicator function, $C_{k}$ is the set of indices of items assigned to cluster $k$, and $y^{(i)}$ is the class label of embedding $\mathbf{z}^{(i)}$.
The cluster purity for this partitioned embedding space is $57.7\%$.
For this experiment, we use $K$-means clustering given its simplicity but are aware that a more sophisticated clustering algorithm, catered to the specific data, might yield better results. 
%Knowing that $K$-means struggles in handling high dimensional data and therefore applying dimensionality reduction before clustering or employing a more sophisticated unsupervised clustering technique might yield better clusters.
Nevertheless, each word segment can now be labelled with a cluster ID (0 to 699) corresponding to the cluster to which its AWE is assigned.   
%For sanity checking, we assign the word label to all items in each cluster to most frequent item.
%This is only for visualisation where no word labels are used during this process.
%After the clustering, each word is assigned the cluster ID to which it belong as word label.
We now essentially have an annotated speech corpus, where the word labels are numbers instead of written words.


%Given that the word itself is not considered but rather its occurrence related to surrounding items, we can train a normal word embedding model in a similar fashion.




%In the next step, we apply k-means clustering to the vector space containing the AWE of all the spoken word segment in the training data.
%The clustering method should distinguish between the AWE that belong to the same word type and those that are from another word type.
%I.e, it should assign embeddings to the same cluster if they are relatively closer to one another than from other embeddings.
%Form a visual perception, we can clearly see some of these clusters, however some of them are more spread out and overlap, which makes it difficult for clustering methods to assign to the correct cluster.
%The result after applying k-means are illustrated on the right of  Figure~\ref{fig:semantic_clustered} where the colours indicate the different clusters.
%We note that there are embeddings from the same word type that belong to multiple embeddings.
%The embeddings of x number of word types are assigned to x different clusters, almost all the available clusters, even if it is just one embedding.
%This goes to show that applying K-means on the high dimensional data is not effective, caught in the curse of dimensionality.



%We calculate the purity of x\%.




\subsection[Semantic embeddings using Skip-gram]{Semantic Embeddings Using Skip-Gram}
\label{ssec:semantic_skipgram}



%\begin{figure}[!b]
%	\centering
%	\centerline{\includegraphics[width=0.65\linewidth]{semantic/figures/cluster_mean_dist.pdf}}
%	\caption{Given an acoustic embedding $\mathbf{z}$ (assigned to cluster no. 3), instead of using a one-hot encoded input $\mathbf{x} = \{0, 0, 1, 0, \cdots, 0\}$, the value at each index is set using Equation~\ref{eqn:semantic_soft_label}, for example, $\mathbf{x} = \{0.03, 0.8, 0.9, 0.05, \cdots, 0.01\}$. Note that the values at index 2 and 3 are the highest given that $\mathbf{z}$ is the closest to cluster means $\mathbf{c}_2$ and $\mathbf{c}_3$. Black squares indicate cluster means.}
%	\label{fig:semantic_cluster_mean_dist}
%\end{figure}


%\begin{figure}[!t]
%	\centering
%	\centerline{\includegraphics[width=0.99\linewidth]{semantic/figures/distribution_semantic_marked.pdf}}
%	\caption{t-SNE visualisations of semantic embeddings produced by the Skip-gram model using the soft labelling approach. The word label given alongside the cluster IDs are only for evaluation purposes and was not used during training.} 
%	\label{fig:semantic_id_embeddings}
%\end{figure}

%We reimplement the skip-gram model of~\citet{mikolov_distributed_2013} described in Section~\ref{sec:semantic_skipgram}.


We train a Skip-gram model (Section~\ref{sec:semantic_skipgram}) using the unknown word labels (cluster IDs) as training data.
Our training setup is similar to the setup of \citet{mikolov_efficient_2013} (discussed in Section~\ref{sec:semantic_background}) where we use one-hot encoded embeddings as input and target outputs.
A non-zero index correspond to the index of the cluster ID in the vocabulary set.
The only difference is that the vocabulary consists of numbers instead of written words.
%This training configuration is the same as described in Section~\ref{sec:semantic_skipgram} where the vocabulary consists of numbers instead of written words.
Preliminary results showed multiple groups of semantically related word embeddings scattered across the entire embedding space.
%since the model treats each cluster ID as a unique word even though multiple cluster IDs may represent the same word type. 
Using the cluster IDs as hard labels to train a Skip-gram model prevents the model from accurately capturing the semantic relationship between word segments because of the following:
Firstly, acoustic embeddings representing different word types that are assigned to the same cluster will have identical word labels and will be interpreted as the same spoken word by the model.   
Secondly, given that acoustic embeddings representing the same word type are assigned to multiple clusters, spoken word segments from the same word type have different labels and therefore be interpreted as different words by the model.
%Secondly, for each word type, instead of only appearing once in the vocabulary, because the clustering process clusters the group of the same word types into multiple clusters, there may exist multiple IDs representing the same word type.
%Both these  will make it more difficult for the word embedding model to properly learn the meaningful relationship between word segments.

%Preliminary experiments showed that using one-hot encoded embeddings for word representations used as input and output values, results in multiple semantically related groups scattered across the entire embedding space.

We therefore alternatively follow a soft labelling approach where, instead of using one-hot encoded input and outputs, we set the value at each index as a function of the distance between the acoustic embedding and every cluster mean. 
Given an acoustic embedding $\mathbf{z}$ and cluster mean $\mathbf{c}_i$, the value at index $i$ is calculated as follows:
%\begin{equation}
%	d_{i} = \text{exp} \left( \frac{1}{\sigma^2} \lVert \mathbf{z} - \mathbf{c}_i \rVert \right)
%	\label{eqn:semantic_soft_label}
%\end{equation}
where $\sigma$ is set to $0.5$ by performing qualitative analysis on a small subset of resulting embeddings.
Figure~\ref{fig:semantic_cluster_mean_dist} illustrates the soft labelling approach.
We use a non-linear scaling approach to assign more weight on embeddings closer to the target embedding $\mathbf{z}$. If another embedding is exponentially closer to the target embedding, it most likely belongs to the same word type but was assigned to a different cluster.
Accordingly, the soft input vector allows multiple rows in weight matrix $\mathbf{W}_1$ to update for a single training example.


%Instead, for each embedding, we calculate the distance between every cluster's mean, then set the value of vector with dim $V$ at index to distance.
%By doing so we use a soft labelling approach for each embedding.
We again train a Skip-gram model, this time using the soft labels as input and output vectors, instead of the hard one-hot vectors.
Figure~\ref{fig:semantic_id_embeddings} show the t-SNE visualisation of the resulting embeddings from which we observe two things.
%Embeddings representing each cluster are displayed in Figure~\ref{fig:semantic_id_embeddings} from which we observe two things.
Firstly, embeddings from different clusters that represent the same word type appear close to each other, caused by using soft-labelled input vectors instead of one-hot vectors.
Secondly, embeddings from clusters that represent different words but with similar meaning are in close proximity.
For example, the embeddings of clusters representing the words ``young'' and ``little'', and ``water'' and ``ocean", appear in a similar context and therefore have similar embeddings.

Given an unseen spoken word segment, we can apply the same multilingual AWE model, identify the nearest cluster mean and assign the embedding to a specific cluster.
The cluster ID to which the embedding is assigned can then be used to identify the semantic embedding in the $\mathbf{W}_1$ matrix, where the row at cluster index is the semantic representation.
%To find semantically related words we can perform a nearest neighbour search to find nearest embeddings by calculating the distance between their vectors.


%For a new input, we produce the AWE and determine to which class it belongs, then use the cluster ID as index in the $\mathbf{W}_1$ matrix. 

%\begin{figure}[!t]
%	\centering
%	\centerline{\includegraphics[width=0.99\linewidth]{semantic/figures/word_labels_semantic_tsne_marked.pdf}}
%	\caption{t-SNE visualisation of word embeddings produced by training a Skip-gram model on true word labels of speech segments, using one-hot encoded vector representations as input and outputs.} 
%	\label{fig:semantic_word_embeddings}
%\end{figure}

We perform a sanity check where we use the transcriptions of the spoken captions to train a Skip-gram model.
In other words, we train a Skip-gram model using true word labels instead of cluster IDs.
We follow the same setup as \citet{mikolov_efficient_2013} (described in Section~\ref{sec:semantic_skipgram}). 
Figure~\ref{fig:semantic_word_embeddings} shows the semantic embeddings for the same evaluation words used previously.
Note, each word label has a unique representation, given that the vocabulary only contains a single instance of each word compared to multiple labels (cluster IDs) representing the same word in Figure~\ref{fig:semantic_id_embeddings}.
Comparing Figure~\ref{fig:semantic_id_embeddings} to Figure~\ref{fig:semantic_id_embeddings}, we observe a similar organisation of embeddings.
For example, the embeddings of ``water" and ``ocean", and ``little" and ``young" are close to each other, similar to Figure~\ref{fig:semantic_id_embeddings}.

From Figure~\ref{fig:semantic_id_embeddings} and Figure~\ref{fig:semantic_word_embeddings} we can conclude that the three-step framework succeeds in learning meaningful representations containing semantic information, with limited supervision.






%An example setup before training the Skipgram is shown in Figure~\ref{}.
%The text corpus is essentially a sequence of numbers corresponding to cluster IDs.
%Instead of using one-hot encoding where the index of the word in the vocabulary is set to one, and the rest zeros, we calculate the distance between the mean of the input word and every other mean and use that as value at each index. 


%We use a window size of 2.
%Parameters are update with different weights according to the frequency of words.
%We update the weights using cross-entropy loss.

%The hidden layer as shown in Figure X, represents the word embedding for each word label.
%If we apply dimensionality reduction technique and plot the word embeddings in Figure X.




%An example setup before training the Skipgram is shown in Figure~\ref{}.
%The text corpus is essentially a sequence of numbers corresponding to cluster IDs.
%Instead of using one-hot encoding where the index of the word in the vocabulary is set to one, and the rest zeros, we calculate the distance between the mean of the input word and every other mean and use that as value at each index.



%We use a window size of 2.
%Parameters are update with different weights according to the frequency of words.
%We update the weights using cross-entropy loss.
%
%The hidden layer as shown in Figure X, represents the word embedding for each word label.
%If we apply dimensionality reduction technique and plot the word embeddings in Figure X.
%
%For a new input, we produce the AWE and determine to which class it belongs, then assign 
%
%
%An example setup before training the Skipgram is shown in Figure~\ref{}.
%The text corpus is essentially a sequence of numbers corresponding to cluster IDs.
%Instead of using one-hot encoding where the index of the word in the vocabulary is set to one, and the rest zeros, we calculate the distance between the mean of the input word and every other mean and use that as value at each index. 
%
%
%We use a window size of 2.
%Parameters are update with different weights according to the frequency of words.
%We update the weights using cross-entropy loss.
%
%The hidden layer as shown in Figure X, represents the word embedding for each word label.
%If we apply dimensionality reduction technique and plot the word embeddings in Figure X.
%
%For a new input, we produce the AWE and determine to which class it belongs, then assign 
%


%\subsection{Semantic word embeddings}[Semantic word embeddings]
%The objective of the skip-gram model is to learn word representations that is useful for predicting neighbouring words in a sentence.
%The model tries to predict surrounding words (context words) given a target word (source word).
%%Formally, given a sequence of training words w1, w2, wT, skipgrams model learns to minim
%
%
%Consider the following example sentence: ``he quick brown fox jumps over the lazy do". 
%The model tries to predict the context vectors [quick, fox] given target word ‘brown’ or [the, brown] given target word ‘quick’ and so on.
%
%
%
%
%We then assign a the cluster label as the word label for the word segment to which the embedding belong.
%A normal skipgram model can be trained by using the cluster labels as word labels, however,
%because of the variance in items in the corpus, some classes have many items and other much less.
%Consequently, some embeddings that belong to the same word type belong to different clusters and therefore assigned different cluster labels which will be treated as complete different words,
%Preliminary experiments showed that training the skipgram using one-hot vectors as input and targets, results in semantically groups scattered across the embedding space.
%To mitigate this effect, instead of using the hard labelling one-hot vector as input and target, we calculate the distance between an embedding and every cluster mean to replace the one one vector.
%This would allow multiple parameters to update.
%For example, [123, 42, 341] where 123 and 341 belong top the same word type.
%Instead of having vector [1, 0, 0], only allowing the first row of the word embedding matric to update, we have [0.9, 0,001, 0.8] allowing both rows to update to push these embeddings in the same direction. 





==> semantic/methodology.tex <==
\mysection{Proposed approach}{Proposed Approach}
\label{sec:semantic_methodology}


\begin{figure}[!b]	
	\centering
	\centerline{\includegraphics[width=\linewidth]{semantic/figures/method.pdf}}
	\caption{Illustration of step 1 and 2 in the framework we propose, showing how unknown word labels are assigned to unlabelled speech segments.}
	\label{fig:semantic_method}
\end{figure}

%In this chapter we propose a three-step framework to produce acoustic-semantic embeddings.
%Here we provide a high-level overview of what each step involves, partly illustrated in Figure~\ref{fig:semantic_method}. 
In this section, we provide a high-level overview of the three-step framework we propose to produce acoustic-semantic embeddings, partly illustrated in Figure~\ref{fig:semantic_method}.
%The three-step framework we follow for producing acoustic-semantic embeddings are partly illustrated in Figure~\ref{fig:semantic_method}.

% of the systematic approach we follow to map variable-duration spoken word segments to fixed-dimensional representations that reflect the underlying meaning of those words as they appear in the context with other words.
%During this process we only use speech and minimal supervision (specified).
%This method can be divided into three main processes as illustrated in Figure~\ref{fig:semantic_method}.
%Firstly, a speech corpus is segmented into isolated speech segments.
\textbf{Step 1.} An unlabelled speech corpus is segmented into isolated word segments using true word boundaries obtained from forced alignments. 
Following the multilingual training strategy as described in Section~\ref{ssec:multilingual}, an AWE model can be applied to any unseen zero-resource language.
Therefore, we apply a pretrained multilingual AWE model to each unknown word segment to produce embeddings only reflecting the acoustic similarity between word segments.

Note, using true word boundaries is a form of supervision. In the zero-resource setting where word boundaries are not available, an unsupervised segmentation algorithm can be used instead, making this step fully unsupervised. For now, we use true word boundaries to simplify our experiment since unsupervised segmentation is a difficult problem on its own.
%Note, these embeddings only reflect the acoustic similarity between speech segments.  
%A pretrained multilingual AWE model is then applied to each speech segments to produce embeddings that reflect the acoustic similarity of the speech segments (embeddings of the same word type should be more similar to each other than to embeddings from different word types).
%The work of previous chapters revolved around this concept.

\textbf{Step 2.} An unsupervised clustering algorithm is applied to the acoustic embedding space that assigns each embedding to one of $K$ clusters.
The goal is to group together embeddings from the same unknown word type given that AWEs from the same unknown word type should be more similar than embeddings from different word types.
%An unsupervised clustering algorithm is applied to the acoustic embedding space that aims to distinguish between embeddings from the same and different word types (embeddings from the same unknown word type should be more similar than embeddings from different word types) and group them accordingly.
%An unknown word label is then assigned to each word segment corresponding to the cluster ID to which its embedding is assigned to.  
Subsequently, a word segment is labelled with the cluster ID to which its AWE is assigned. 
%representative of the cluster to which the AWE of the segment belong.
This process can be interpreted as unsupervised labelling of the speech corpus, where each word segment now have an unknown word label (cluster ID).
%This is similar to the setup for training textual word embedding model similar as ~\citet{mikolov_distributed_2013} where the text corpus is unknown words (cluster IDs) instead of actual words from the English vocabulary.

\textbf{Step 3.} Use the Skip-gram model of \citet{mikolov_efficient_2013} (Section~\ref{sec:semantic_skipgram}) to learn semantic embeddings, using unknown word labels (cluster IDs) instead of true word labels.
Since the word itself is not important, but rather the context in which it occurs with other words, there is no difference in the label used for representing a word from the models perspective.
Importantly, if the clustering algorithm were able to group the acoustic embeddings perfectly, where word segments from the same word type are labelled with the same cluster ID, there would be no difference between using the true word labels of written text or the unknown word labels.
However, the AWE model and unsupervised clustering algorithm do not allow for such accurate labelling of word segments.
%The result thereof and how we attend to them are discussed in the following sections.


%Next, we apply a clustering algorithm to the acoustic embedding space that assigns each AWE to a group.
%The goal is to distinguish between embeddings that belong to different word types, by grouping embeddings from the same word type in a common group.

%After clustering the acoustic embedding space, the speech segment are labelled with a number according to the cluster to which their acoustic embedding belong.

%Details regarding the model is described in the following section.



%To use the skipgram model, we need to assign labels to each speech segment, without using word labels.




%word segments are extracted and embedded to fixed-dimensional representations, using a multilingual AWE model where no data of the target language have been seen during training.
%After embedding each segment with the same AWE model, we apply a clustering technique, dividing the embedding space in different classes.








